Optimal uncertainty relations in a modified Heisenberg algebra

Various theories that aim at unifying gravity with quantum mechanics suggest modifications of the Heisenberg algebra for position and momentum. From the perspective of quantum mechanics, such modifications lead to new uncertainty relations which are thought (but not proven) to imply the existence of a minimal observable length. Here we prove this statement in a framework of sufficient physical and structural assumptions. Moreover, we present a general method that allows to formulate optimal and state-independent variance-based uncertainty relations. In addition, instead of variances, we make use of entropies as a measure of uncertainty and provide uncertainty relations in terms of min- and Shannon entropies. We compute the corresponding entropic minimal lengths and find that the minimal length in terms of min-entropy is exactly one bit.

==> pix/convex.tex <==
%% Creator: Inkscape 0.91_64bit, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'convex.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{834.33982068bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
    \begin{picture}(1,0.94247057)%
    \put(0,0){\includegraphics[width=\unitlength,page=1]{convex.pdf}}%
    \put(0.3103449,0.58652265){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\Gamma(\mathcal{U})$}}}%
    \put(-0.0703449,0.88652265){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\Delta p$}}}%
    \put(0.2974103,0.3650547638){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\Gamma(\mathcal{U}_{lc})$}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=2]{convex.pdf}}%
    \put(0.92652265,-0.0303449){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\Delta x$}}}%
    \put(0.2503449,0.8752265){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\lambda=1$}}}%
    \put(0.183449,0.1782265){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\lambda=0$}}}%
    \put(-0.0703449,0.0652265){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$u(0)$}}}%
    \put(-0.0703449,0.7052265){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\frac{u(\lambda)}{1-\lambda}$}}}%
    \end{picture}%
\endgroup%


==> pix/dxdp.tex <==
%% Creator: Inkscape 0.48.3.1, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'dxdp.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{533.86699219bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,1.00298392)%
    \put(0,0){\includegraphics[width=\unitlength]{dxdp.pdf}}%
    \put(0.19662651,0.72055525){\makebox(0,0)[lb]{\smash{harmonic oscillator ground states} }}%
   % \put(0.53594832,0.28728105){\makebox(0,0)[lb]{\smash{no harmonic oscillator ground states}}}%
       \put(0.16897475,0.43688634){\makebox(0,0)[lb]{\smash{maximally localized states}}}%
    \put(0.63768146,0.80914576){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{\huge{$\mathcal{U}$}}}}%
    \put(-0.02,0.9){\makebox(0,0)[lb]{\smash{$\Delta x$}}}%
    \put(0.95,0.05){\makebox(0,0)[lb]{\smash{$\Delta p$}}}%
    \put(0.0,0.2897475){\makebox(0,0)[lb]{\smash{$\beta$}}}%
      \end{picture}%
\endgroup%


==> pix/entroucr.tex <==
%% Creator: Inkscape 0.48.3.1, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'entroucr.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{399.83540039bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.83288918)%
    \put(0,0){\includegraphics[width=\unitlength]{entroucr.pdf}}%
    \put(0.42848099,0.56288661){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{\footnotesize minimal position entropy}}}%
    \put(0.55743848,0.62756002){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{\footnotesize  maximal position entropy}}}%
    \put(0.55844902,0.44969997){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{\footnotesize  maximally localized states}}}%
    \put(0.08387717,0.76601084){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$h_p$}}}%
    \put(0.84642855,0.16759253){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$h_x$}}}%
  \end{picture}%
\endgroup%


==> pix/hmin.tex <==
%% Creator: Inkscape 0.48.3.1, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'hmin.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{529.7890625bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.50126746)%
    \put(0,0){\includegraphics[width=\unitlength]{hmin.pdf}}%
    \put(-0.00053823,0.48946294){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$h^p_\infty$}}}%
	\put(0.01053823,0.28946294){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\Gamma_{\min}^{\infty}$}}}%
    \put(0.96058307,0.27805805){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$h^x_\infty$}}}%
    \put(0.48099733,0.1029953){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{\large$\mc{U}_{h_\infty}$}}}%
  \end{picture}%
\endgroup%


==> pix/positions2.tex <==
%% Creator: Inkscape 0.48.3.1, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'positions2.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{539bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.62152134)%
    \put(0,0){\includegraphics[width=\unitlength]{positions2.pdf}}%
    \put(0.6641258,0.29811677){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{minimal variance}}}%
    \put(0.64492753,0.57246377){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{small entropy}}}%
    \put(0.07246377,0.58695653){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{highest peak}}}%
    \put(0.98789987,0.03381818){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$x$}}}%
    \put(0.46013181,0.6363961){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\mathbb{P}(x)$}}}%
  \end{picture}%
\endgroup%

